Markov Process-Based Graph Convolutional Networks for Entity Classification in Knowledge Graphs

Despite the vast amount of information encoded in Knowledge Graphs (KGs), information about the class affiliation of entities remains often incomplete. Graph Convolutional Networks (GCNs) have been shown to be effective predictors of complete information about the class affiliation of entities in KGs. However, these models do not learn the class affiliation of entities in KGs incorporating the complexity of the task, which negatively affects the models prediction capabilities. To address this problem, we introduce a Markov process-based architecture into well-known GCN architectures. This end-to-end network learns the prediction of class affiliation of entities in KGs within a Markov process. The number of computational steps is learned during training using a geometric distribution. At the same time, the loss function combines insights from the field of evidential learning. The experiments show a performance improvement over existing models in several studied architectures and datasets. Based on the chosen hyperparameters for the geometric distribution, the expected number of computation steps can be adjusted to improve efficiency and accuracy during training.

==> tables/datasets_rgcp.tex <==
\begin{table}[!ht]
\centering
  \caption{Statistics of FB15kET and YAGO43kET Datasets}
  \label{tab:datasets_entyp}
  \begin{center}
  \begin{tabular}{lrr}
    \toprule
    \textbf{Dataset}   & \textbf{FB15kET} & \textbf{YAGO43kET} \\
    \midrule
    \textbf{\#Entities} & 14,951 & 42,335\\
    \textbf{\#Relations} & 1,345 & 37 \\
    \textbf{\#Types} & 3,584 & 45,182 \\
    \textbf{\#Train.triples} & 483,142 & 331,686\\
    \textbf{\#Train\_ET} & 136,618 & 375,853\\
    \textbf{\#Valid\_ET} & 15,848 & 43,111\\
    \textbf{\#Test\_ET} & 15,847 & 43,119\\
    \bottomrule
  \end{tabular}
\end{center}
\end{table}

==> tables/hyperparameter-setting.tex <==
\begin{table}[t!]
  \caption{Hyperparameters for MPERL+R-GCN}
  %\caption{Details of the hyperparameters for MPERL+R-GCN}
  \label{tab:hyparameter}
  \begin{center}
  {\scriptsize
    \begin{tabular}{lcccc}
      \toprule
      \textbf{Hyperparameter}    & \textbf{AIFB}  & \textbf{MUTAG} & \textbf{BGS} & \textbf{AM} \\
      \midrule
      Hidden Dimension & 16 & 16 & 16 & 10 \\
      Number of bases & 0 & 45 & 45 & 55 \\
      Learning Rate & 0.01 & 0.005 & 0.005 & 0.005 \\
      Dropout & 0 & 0.3 & 0.2 & 0 \\
      Weight Decay & 5e-5 & 1e-3 & 5e-3 & 5e-5 \\
      Epochs & 30 & 10 & 30 & 55 \\
      \bottomrule
    \end{tabular}
  }
  \end{center}
\end{table}
